The Spectrum of Fisher Information of Deep Networks Achieving Dynamical Isometry

The Fisher information matrix (FIM) is fundamental to understanding the trainability of deep neural nets (DNN), since it describes the parameter space's local metric. We investigate the spectral distribution of the conditional FIM, which is the FIM given a single sample, by focusing on fully-connected networks achieving dynamical isometry. Then, while dynamical isometry is known to keep specific backpropagated signals independent of the depth, we find that the parameter space's local metric linearly depends on the depth even under the dynamical isometry. More precisely, we reveal that the conditional FIM's spectrum concentrates around the maximum and the value grows linearly as the depth increases. To examine the spectrum, considering random initialization and the wide limit, we construct an algebraic methodology based on the free probability theory. As a byproduct, we provide an analysis of the solvable spectral distribution in two-hidden-layer cases. Lastly, experimental results verify that the appropriate learning rate for the online training of DNNs is in inverse proportional to depth, which is determined by the conditional FIM's spectrum.

==> comments.tex <==
\begin{comment}
(i)直交初期化 

- Provable Benefit of Orthogonal Initialization in Optimizing Deep Linear Networks

https://openreview.net/forum?id=rkgqN1SYvr
線形深層でのdynamics解析。https://arxiv.org/abs/1312.6120 の理論を精緻化して、収束速度を定量的に解析

- Information Geometry of Orthogonal Initializations and Training 

https://openreview.net/forum?id=rkg1ngrFPr
訓練中も直交制約を課す実験論文。高速な収束。ただし、FIMの最大固有値は増加するらしい。
NTK regimeを外れていると思われる。


(ii) FIMを単位行列に近づける

- http://proceedings.mlr.press/v22/raiko12.html

skip-connectionを使う

- http://papers.nips.cc/paper/5953-natural-neural-networks

各学習ステップで$$E[hh^\top]$$が単位行列になるように正規化 ($$\delta \delta^\top$$は無視)


\subsection{Linear}
linear theoretical dynamics: ICLR 2020
%設定は違うけど、consistent.
%non-linearでもいけた
% introよりはこっちのほうが良いかも。
%%%% < ---- training dynamics (orthogonal + NTK) ICLR2020 ?
%%%% Information Geometry of Orthogonal Initializations and Training
%%%% linear vs non-linear

\subsection{Neural Tangent Kernel}

\paragraph{NTK}
% ---> intro からもってきた　
The neural tangent kernel \cite{Jacot2018NeuralNetworks} (NTK) is a dual of FIM, which describes the training dynamics of DNN. \com{Eigenvalues of }
The NTK has spectral distribution except for zero eigenvalues with the FIM. 
%%% <----


Secondly, consider the \emph{neural tangent kernel} $\Theta \in M_{M}(\R) \otimes M_{N}(\R)$ whose $(m,n)$-block is defined  as 
\begin{align}
    \Theta(m,n)  =  \frac{1}{N}\pp{f_{\theta}(x(m))}{\theta}  \pp{f_{\theta}(x(n))}{\theta}^T.
\end{align}
Then $\hat{F}$ and $\Theta$ share non-zero eigenvalues; denote  each spectral distribution by  $\mu_{\hat{F}}$ and $\mu_\Theta$, then
\begin{align}
\mu_{\hat{F}}  =  (1- \frac{1}{LM}) \delta_0 + \frac{1}{LM}\mu_\Theta.
\end{align}


\begin{rmk}(Neural Tangent Kernel)\cite{Jacot2018NeuralNetworks} 
\begin{align}
    \Theta(x, x^\prime) =  \frac{1}{N}\pp{f_{\theta}(x)}{\theta}  \pp{f_{\theta}(x^\prime)}{\theta}^T.
\end{align}
\end{rmk}

\end{comment}


%To approximately achieve  dynamical isometry,  we assume that the spectral distribution of $JJ^T$ 
%converges to  a compactly supported probability distribution as $L \to \infty$.
%Note that we choose appropriate $\sigma_\ell$ and $\phi_\ell$ ($\ell=1, \dots, L$)  for each $L$. 
%Therefore, the notation such as $\sigma_\ell^{(L)}$  prevents misunderstanding, but since this notation is cumbersome, we omit the symbol $(L)$.
%Recall that we use the orthogonal initialization since Gaussian initialization breaks dynamical isometry  as the deep limit $L \to \infty$ \cite{Pennington2018emergence}.

